Graph Alignment Topology as an Inductive Bias for Grounding Detection

Large Language Models (LLMs) are optimized to produce distributionally plausible continuations rather than to explicitly verify whether generated propositions are entailed by source documents. This inductive bias enables generalization, but it does not encode whether responses are grounded with respect to a reference. These issues limit the use of LLMs in domains where strict factual correctness is crucial, such as clinical decision support. Existing hallucination detection approaches improve factuality through retrieval augmentation, self-consistency, or claim verification, but generally do not learn directly over alignment topology. To leverage alignment topology as an inductive bias, we construct aligned bipartite graphs between reference information and LLM outputs and train a graph neural network (GNN) to model alignment structure using message passing. The method achieves state-of-the-art results on four diverse hallucination and question-answering datasets, outperforming all compared methods, including foundational LLMs such as GPT-4o.

==> makefile <==
# Paul Landes - 6/20/2018
# export version makefile
# https://github.com/plandes/zenbuild
#
# To build you need:
#   - Latex2e
#   - pdflatex
#   - either bibtex or biber if `zenbiber` is present
#   - GNU make


## setup

# binaries
TEX_LATEX_CMD =	pdflatex "$(TEX).tex"
BIBTEX=		bibtex
BIBER=		biber
BIB_FILE=	$(wildcard *.bib)

# files
TEX=		main
TEX_LATEX_FILE=	$(TEX).tex
TEX_PDF_FILE=	$(TEX).pdf
TEX_FINAL_RUNS =2


## targets

# default target
all:		pdf

# build information
.PHONY:		info
info:
		@echo "name: $(TEX)"
		@echo "tex: $(TEX_LATEX_FILE)"
		@echo "pdf: $(TEX_PDF_FILE)"
		@echo "bib-file: $(BIB_FILE)"

# build the PDF file
.PHONY:		pdf
pdf:		$(TEX_PDF_FILE)

$(TEX_PDF_FILE):	$(TEX_LATEX_FILE)
		$(TEX_LATEX_CMD)
		if [ -f "$(BIB_FILE)" ] ; then \
			if [ -f zenbiber ] ; then \
				$(BIBER) $(TEX) ; \
			else \
				$(BIBTEX) $(TEX) ; \
			fi \
		fi
		for i in `seq $(TEX_FINAL_RUNS)` ; do \
			$(TEX_LATEX_CMD) $(TEX).tex ; \
		done

# clean a used build
clean:
		rm -f *.pdf *.out *.aux *.log *.bbl *.bcf *.blg \
			*.upa *.upb *.xml *.toc *.nav *.snm

